Chemical short range order obtained from the atomic pair distribution function

Many crystalline materials show chemical short range order and relaxation of neighboring atoms. Local structural information can be obtained by analyzing the atomic pair distribution function (PDF) obtained from powder diffraction data. In this paper, we present the successful extraction of chemical short range order parameters from the x-ray PDF of a quenched Cu_3Au sample.

==> elements.tex <==
%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen

\renewcommand{\Title}{Chemical short range order obtained from the atomic pair
                      distribution function}
\renewcommand{\AuthorsComplete}{Th. Proffen$^{I*}$, V. Petkov$^{II}$,
                                S.J.L. Billinge$^{II}$, T. Vogt$^{III}$}

\renewcommand{\CorrespondenceAuthor}{(e-mail: tproffen@lanl.gov)}

\renewcommand{\InstitutionOne}
      {Los Alamos National Laboratory, LANSCE-12, MS H805, Los Alamos, NM 87545, USA}

\renewcommand{\InstitutionTwo}
      {Department of Physics and Astronomy, Michigan State University, East Lansing,
       MI 48824-1116, USA}

\renewcommand{\InstitutionThree}
      {Physics Department, Brookhaven National Laboratory, Upton, NY 11973, USA}

\renewcommand{\InstitutionFour}{}    %will appear under IV
\renewcommand{\InstitutionFive}{}    %will appear under V
\renewcommand{\InstitutionSix}{}     %will appear under VI

\renewcommand{\SayThanks}{}

\renewcommand{\Abstract}
{
%
  Many crystalline materials show chemical short range
  order and relaxation of neighboring atoms. Local structural
  information can be obtained by analyzing the atomic pair
  distribution function (PDF) obtained from powder diffraction data.
  In this paper, we present the successful extraction of chemical
  short range order parameters from the x-ray PDF of a quenched
  Cu$_3$Au sample.
%
} % includes the full abstract in English!


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Paperreceived}{xxx xx, 2001}  % date only; format: April 23, 1998
\renewcommand{\Paperaccepted}{xxx xx, 2001}      % date only; format: April 24, 1998
\setcounter{Papervolume}{216}                    % publisher: volume number here
\setcounter{page}{000}                           % publisher: pagenumber here

\renewcommand{\Authors}{Th. Proffen, V. Petkov, S.J.L. Billinge, T. Vogt}

\renewcommand{\cleanTitle}{}   % only needed to eliminate additions from Title
                               % like footnotes etc. for databank purposes
\renewcommand{\shortAuthors}{Proffen et al.} % only needed for headings; else = Authors
\renewcommand{\shortTitle}{Chemical short range order obtained from the atomic pair
                           distribution function}
                               % only needed for headings; else = cleanTitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\endinput

